PF-LRM: Pose-Free Large Reconstruction Model for Joint Pose and Shape Prediction

We propose a Pose-Free Large Reconstruction Model (PF-LRM) for reconstructing a 3D object from a few unposed images even with little visual overlap, while simultaneously estimating the relative camera poses in ~1.3 seconds on a single A100 GPU. PF-LRM is a highly scalable method utilizing the self-attention blocks to exchange information between 3D object tokens and 2D image tokens; we predict a coarse point cloud for each view, and then use a differentiable Perspective-n-Point (PnP) solver to obtain camera poses. When trained on a huge amount of multi-view posed data of ~1M objects, PF-LRM shows strong cross-dataset generalization ability, and outperforms baseline methods by a large margin in terms of pose prediction accuracy and 3D reconstruction quality on various unseen evaluation datasets. We also demonstrate our model's applicability in downstream text/image-to-3D task with fast feed-forward inference. Our project website is at: https://totoro97.github.io/pf-lrm .

==> 03_method_backup_kai.tex <==
\section{Method}
\label{sec:method}


\begin{figure} \label{fig:method}
\includegraphics[width=0.96\textwidth]{figures/method.png}
\caption{\kz{Suggested by Zexiang: in the figure, show predicted points for this example instead of colored tokens}}
\end{figure}

\subsection{Single-stream Transformer}
We apply tokenization to both the input images and the triplane representation. We then use the self-attention mechanism to model the information exchanges among these tokens. Besides reconstructing the triplane NeRF, we also aim to predict the camera poses of all source views relative to a reference view. To equip the set-based transformer model with a sense of context (reference view),  we introduce two additional view encoding vectors — one for the reference view and another for all source views, for modulating the image patch tokens.  


\noindent \textbf{Image tokenization and view encoding}. We use the pretrained DINO\kz{TODO: cite} Vision Transformer to tokenize our input images. DINO uses a patch size of 16x16 and 16-layer transformer of width 768. Each input image of resolution HxW is tokenized into H/16xW/16 tokens of 768-dim. 

Our approach utilizes two distinct 768-dimensional learnable features which serve as view encoding vectors. One vector is used to modulate the tokens corresponding to the reference image, while the other vector is applied to modulate the patch tokens of each individual source view. This architectural design essentially aids the transformer model in distinguishing between tokens associated with the reference view and those related to the various source views. As our objective is to predict relative poses, the tokens from the reference view function as contextual references for the source view tokens. Consequently, we leverage the view encoding mechanism to effectively mark these vital context tokens.

\kz{Add modulation equation here}

\noindent \textbf{Triplane tokenization}. We directly tokenize our triplane of shape 3xH'xW'xC' (where H',W' are spatial resolution and C' is the channel dimension) into 3xH'xW' tokens. To get these tokens, our transformer model learns to translate 3xH'xW' learnable triplane tokens of 768-dim into the target triplane tokens through self-attention over all image tokens and triplane tokens. We then use a MLP to change the token dimension from 768 to C'. \kz{mention triplane upsampling here}

To predict the NeRF density and colors at each 3D point, we use another MLP to convert the trilinearly interpolated triplane feature; we then perform volume rendering to get the final color image. This MLP is shared for all predicted triplanes and trained together with the transformer.

\noindent \textbf{Variable number of input views}. Our model naturally supports variable number of input views, thanks to the design choices of sharing one view encoding vector among all source views and employing the self-attention architecture. Adding/reducing number of images is just like increasing/shortening sentences in GPT-style language models.

\subsection{Differentiable PnP Solver}
We use the differentiable PnP solver proposed by \kz{Add citation} to solve for camera poses from a set of 3D-2D correspondences (3D: per-patch predicted point, 2D: per-patch pixel center). \kz{briefly explain how the differentiable PnP solver works here}

\subsection{Loss functions}
\noindent \textbf{Point loss}. We use a MLP to predict a surface point for each patch token output by the transformer. The predicted surface point is supervised to align with volume-rendered surface point from the predicted triplane NeRF corresponding to the ray of the patch center pixel. To account for non-object patch centers, we also use the accumulated transmittance to weigh the per-patch point loss.   

\kz{Add math equations here}

\noindent \textbf{Relative pose loss}. The per-patch predicted points establish a set of 3D-2D correspondences for each view, where for each patch, the predicted 3D point correspond to the center pixel of the patch. We use a differentiable PnP solver to obtain the camera poses, and compare it against ground-truth poses.

\kz{Add math equations here}


\noindent \textbf{Rendering loss}. To supervise the predicted triplane NeRF, we render it from multiple viewpoints using the ground-truth camera poses, and then compute image reconstruction losses, including L2 loss and LPIPS loss, between the renderings and ground-truth images. 

\kz{test if rendering loss using predicted poses is helpful}

\subsection{Implementation details}

\kz{Mention image resolution, triplane resolution, transformer layer and width, rendering resolution, batch size, number of supervision images, number of GPUs, training time}

We train \ourmethod using two different configs, one is a small model and one is a large model.
For the setting of small model (config-S), the number of self-attention layers is 24. The input image resolution is 256, and the output triplane resolution is 64. For NeRF rendering, we uniformly sample 64 points per rays. Training is done on 8 Nvidia A-100 GPUs with xxx days.
For the setting of large model (config-L), the number of self-attention layers is 36. The input image resolution is 512, and the output triplane resolution is 64. For NeRF rendering, we uniformly sample 128 points per rays. Training is done on 128 Nvidia A-100 GPUs with xxx days.
(To add more...)

